Exact solutions for ground effect

"Ground effect" refers to the enhanced performance enjoyed by fliers or swimmers operating close to the ground. We derive a number of exact solutions for this phenomenon, thereby elucidating the underlying physical mechanisms involved in ground effect. Unlike previous analytic studies, our solutions are not restricted to particular parameter regimes such as "weak" or "extreme" ground effect, and do not even require thin aerofoil theory. Moreover, the solutions are valid for a hitherto intractable range of flow phenomena including point vortices, uniform and straining flows, unsteady motions of the wing, and the Kutta condition. We model the ground effect as the potential flow past a wing inclined above a flat wall. The solution of the model requires two steps: firstly, a coordinate transformation between the physical domain and a concentric annulus, and secondly, the solution of the potential flow problem inside the annulus. We show that both steps can be solved by introducing a new special function which is straightforward to compute. Moreover, the ensuing solutions are simple to express and offer new insight into the mathematical structure of ground effect. In order to identify the missing physics in our potential flow model, we compare our solutions against new experimental data. The experiments show that boundary layer separation on the wing and wall occurs at small angles of attack, and we suggest ways in which our model could be extended to account for these effects.

==> figures/potFlow-4.tex <==
 \begin{tikzpicture}[%
trim axis left, trim axis right
]
 \begin{axis}[
  set layers,
ylabel shift = \yshift,
xlabel shift = \xshift,
 width=\fwidth,
 height=0.33333\fwidth,
 at={(0,0)},
scale only axis,
enlargelimits=false,
axis on top,
xlabel={$x$},
ylabel={$y$}]
\addplot graphics[xmin=-1.067,xmax=1.933,ymin=0,ymax=1] {potFlow-4.png};

    \end{axis}
    \end{tikzpicture}

==> sections/lift-asymp.tex <==
\section{Comparison of circulation to asymptotic solutions}
In this section we compare our exact solution for the circulation against two other solutions in the literature. Firstly, the circulation for extreme ground effect ($D \ll 1$) in the thin aerofoil regime ($\alpha \ll 1$) was found by \citeSupp{Widnall1970} as
\begin{align}
    \Gamma & = -\alpha \left( \frac{1}{D}  +\frac{2}{\pi} \log \left(\frac{\pi}{D} \right) + \frac{1}{\pi}\right). \label{Eq:extreme}
\end{align}
Secondly, by using a lumped-vortex method and enforcing the no-flux boundary condition at only a single point, \citeSupp{Katz2001} calculated the circulation as
\begin{align}
    \Gamma & = \pi  \sin(\alpha) \left(\frac{ 1 - \sin(\alpha)/(2 D) + 1/(4 D)^2 }{\sin(\alpha)/(4 D)-1} \right). \label{Eq:plotkin}
\end{align}
In figure \ref{Fig:circ} we compare the solutions  \eqref{Eq:extreme} and \eqref{Eq:plotkin} against our new solution. We see that our new solution agrees well with the asymptotic solution for extreme ground effect \eqref{Eq:extreme}, $0<D<1/4$, for small angle of attack $4^\circ$. As expected, the solutions diverge for larger values of $d$ since the asymptotic solution, \eqref{Eq:extreme}, is inaccurate in all other regimes. Conversely, we obtain excellent agreement with the lumped-vortex method \eqref{Eq:plotkin} in the weak ground effect regime ($D>1$) where that model is accurate.

Our new solution agrees both with extreme and weak ground effect and therefore fills the missing gap between previous models and provides predictions for the circulation which are valid across all ground effect regimes, crucially including the moderate regime where $1/2<D<1$.
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figures/circ}
    \caption{Comparison of circulation from our new solution and other solutions in the literature.}
    \label{Fig:circ}
\end{figure}
